Compact User-Specific Reconfigurable Intelligent Surfaces for Uplink Transmission

Large-scale antenna arrays employed by the base station (BS) constitute an essential next-generation communications technique. However, due to the constraints of size, cost, and power consumption, it is usually considered unrealistic to use a large-scale antenna array at the user side. Inspired by the emerging technique of reconfigurable intelligent surfaces (RIS), we firstly propose the concept of user-side RIS (US-RIS) for facilitating the employment of a large-scale antenna array at the user side in a cost- and energy-efficient way. In contrast to the existing employments of RIS, which belong to the family of base-station-side RISs (BSS-RISs), the US-RIS concept by definition facilitates the employment of RIS at the user side for the first time. This is achieved by conceiving a multi-layer structure to realize a compact form-factor. Furthermore, our theoretical results demonstrate that, in contrast to the existing single-layer structure, where only the phase of the signal reflected from RIS can be adjusted, the amplitude of the signal penetrating multi-layer US-RIS can also be partially controlled, which brings about a new degree of freedom (DoF) for beamformer design that can be beneficially exploited for performance enhancement. In addition, based on the proposed multi-layer US-RIS, we formulate the signal-to-noise ratio (SNR) maximization problem of US-RIS-aided communications. Due to the non-convexity of the problem introduced by this multi-layer structure, we propose a multi-layer transmit beamformer design relying on an iterative algorithm for finding the optimal solution by alternately updating each variable. Finally, our simulation results verify the superiority of the proposed multi-layer US-RIS as a compact realization of a large-scale antenna array at the user side for uplink transmission.

==> TCOM_submission(final)/biographies1.tex <==
\begin{IEEEbiography}[{\includegraphics[trim = 126 315 332 355, clip, width=1in,height=1.25in,keepaspectratio]{fig/KunzanLiu.eps}}]{Kunzan Liu}
has been pursuing the B.E. degree with the Department of Electronic Engineering, Tsinghua University, Beijing, China, since 2018. He joined the Tsinghua National Laboratory for Information Science and Technology (TNList) as a research student in 2020. His research interests include reconfigurable intelligent surface (RIS) and massive MIMO.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[trim = 0 60 0 5,width=1in,height=1.25in,clip,keepaspectratio]{fig/Zijian_Zhang.eps}}]{Zijian Zhang}
(S'20) received the B.E. degree in electronic engineering from Tsinghua University, Beijing, China, in 2020. He is currently working toward the Ph.D. degree in electronic engineering from Tsinghua University, Beijing, China.
His research interests include physical-layer algorithms for massive MIMO and reconfigurable intelligent surfaces (RIS). He has received the National Scholarship in 2019.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/LinglongDai_Photo.eps}}]{Linglong Dai} (M'11-SM'14) received the B.S. degree from Zhejiang University, Hangzhou, China, in 2003, the M.S. degree (with the highest honor) from the China Academy of Telecommunications Technology, Beijing, China, in 2006, and the Ph.D. degree (with the highest honor) from Tsinghua University, Beijing, China, in 2011. From 2011 to 2013, he was a Postdoctoral Research Fellow with the Department of Electronic Engineering, Tsinghua University, where he was an Assistant Professor from 2013 to 2016 and has been an Associate Professor since 2016. His current research interests include reconfigurable intelligent surface (RIS), massive MIMO, millimeter-wave or Terahertz communications, and machine learning for wireless communications.

He has coauthored the book {\it MmWave Massive MIMO: A Paradigm for 5G} (Academic Press, 2016). He has authored or coauthored over 60 IEEE journal papers and over 40 IEEE conference papers. He also holds 19 granted patents. He has received five IEEE Best Paper Awards at the IEEE ICC 2013, the IEEE ICC 2014, the IEEE ICC 2017, the IEEE VTC 2017-Fall, and the IEEE ICC 2018. He has also received the Tsinghua University Outstanding Ph.D. Graduate Award in 2011, the Beijing Excellent Doctoral Dissertation Award in 2012, the China National Excellent Doctoral Dissertation Nomination Award in 2013, the URSI Young Scientist Award in 2014, the IEEE Transactions on Broadcasting Best Paper Award in 2015, the Electronics Letters Best Paper Award in 2016, the National Natural Science Foundation of China for Outstanding Young Scholars in 2017, the IEEE ComSoc Asia-Pacific Outstanding Young Researcher Award in 2017, the IEEE ComSoc Asia-Pacific Outstanding Paper Award in 2018, the China Communications Best Paper Award in 2019, the IEEE Access Best Multimedia Award in 2020, and the IEEE Communications Society Leonard G. Abraham Prize in 2020. He was listed as a Highly Cited Researcher by Clarivate Analytics in 2020.

He is an Area Editor of {\sc IEEE Communications Letters}, and an Editor of {\sc IEEE Transactions on Communications} and {\sc IEEE Transactions on Vehicular Technology}. Particularly, he is dedicated to reproducible research and has made a large amount of simulation codes publicly available.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/Lajos_Hanzo.eps}}]{Lajos Hanzo}
(\url{http://www-mobile.ecs.soton.ac.uk}, \url{https://en.wikipedia.org/wiki/Lajos_Hanzo}) (FIEEE'04) received his 
Master degree and Doctorate in 1976 and 1983, respectively from the 
Technical University (TU) of Budapest. He was also awarded the Doctor of 
Sciences (DSc) degree by the University of Southampton (2004) and 
Honorary Doctorates by the TU of Budapest (2009) and by the University 
of Edinburgh (2015).  He is a Foreign Member of the Hungarian Academy of 
Sciences and a former Editor-in-Chief of the IEEE Press.  He has served 
several terms as Governor of both IEEE ComSoc and of VTS.  He is also a 
Fellow of the Royal Academy of Engineering (FREng), of the IET and of 
EURASIP.
\end{IEEEbiography}

